Learning normal asymmetry representations for homologous brain structures

Although normal homologous brain structures are approximately symmetrical by definition, they also have shape differences due to e.g. natural ageing. On the other hand, neurodegenerative conditions induce their own changes in this asymmetry, making them more pronounced or altering their location. Identifying when these alterations are due to a pathological deterioration is still challenging. Current clinical tools rely either on subjective evaluations, basic volume measurements or disease-specific deep learning models. This paper introduces a novel method to learn normal asymmetry patterns in homologous brain structures based on anomaly detection and representation learning. Our framework uses a Siamese architecture to map 3D segmentations of left and right hemispherical sides of a brain structure to a normal asymmetry embedding space, learned using a support vector data description objective. Being trained using healthy samples only, it can quantify deviations-from-normal-asymmetry patterns in unseen samples by measuring the distance of their embeddings to the center of the learned normal space. We demonstrate in public and in-house sets that our method can accurately characterize normal asymmetries and detect pathological alterations due to Alzheimer's disease and hippocampal sclerosis, even though no diseased cases were accessed for training. Our source code is available at https://github.com/duiliod/DeepNORHA.

==> aux.tex <==



%\subsection{Autoencoder}
 % Se uso una arquitectura de LeNet adaptada para imagenes 3d para reconstruir imagenes

 % A la salida se uso una OC-SVM para clasificar normales de sanos

 % Se probo entrenar con un autoencoder para cada hippocampo

 % Se probo un unico AE capaz de reconstruir ambos hippocampos

 % Se probo espejando la entrada para que los dos hippocampos queden iguales

 % Ademas se probaron dos variantes para agrupar los embedding, resta y concatenacion repectivamente

\subsection{Ablation study}
% Para el caso del siamese encoder se uso el encoder del autoencoder que mejor resultado obtuvo en la tarea anterior

% Para la PH se agrego una capa fully conected a  la salida de los encoder para mapear a otro espacio

% Ademas se probaron 8 diferentes networks previo a la conjuncion de los vectores representativos

\begin{figure}
\centering
\includegraphics[width=1\textwidth]{MICCAI2_2.png}
\caption{A figure caption is always placed below the illustration.
Please note that short captions are centered, while long ones are
justified by the macro package automatically.} \label{fig2}
\end{figure}

We select the following repesentative models for comparison:
\begin{enumerate}
    \item Volume classifier
    \item Asymmetry Index: using the formula in  Z FU
    \item NORHA: this model applied morphological analisis
    \item DCAE: this method applies the deep convolutional autoencoder method to build the one-class clasiffier. The model is trained  by the MSE loss between  the original data and the reconstructions.
    \item DCAE with right hipposcampus flipped: this model is similar to the aforementioned but one of the input is flip
    \item DSVDD with Siamese AE: The model is developed by the proposed method in this paper
    \item DSVDD with Siamese AE and Volume: same strategy but the input contain information of the volume alongside the image  
\end{enumerate}





\subsection{Autoencoder for OCC}
% The result for the different autoencoder are show in table 2 and table 3.
% its noteworthy how in both tables, the AUC increase when only 1 AE is used to reconstruct.

% Explicitly defining the difference between outputs also obtain better values than a mere concatenation of the latent space

\subsection{Ablation analysis}

\subsection{Experiment results}

% \begin{table}[!htb]
%     \begin{minipage}{.5\linewidth}
%       \caption{}
%       \centering
%         \begin{tabular}{c|c|c|c|c|c}
        
%             Arch & No. Enc & Flipp & Oper & AUC & No. param \\
%             \hline
%             LeNet & 2 & - & - & 0.62 & 5.4M \\
%             LeNet & 1 & - & Diff & 0.76 & 2.7M \\
%             LeNet & 1 & - & Concat & 0.71 & 2.7M \\
%             LeNet & 1 & x & Diff & {\bfseries0.99} & 2.7M \\
%             LeNet & 1 & x & Concat & 0.73 & 2.7M \\
%             \hline
%             Enzo & 2 & - & - & 0.58 & 1.1M \\
%             Enzo & 1 & - & Diff & 0.81 & 555K \\
%             Enzo & 1 & - & Concat & 0.72 & 555K \\
%             Enzo & 1 & x & Diff & 0.94 & 555K \\
%             Enzo & 1 & x & Concat & 0.75 & 555K \\
%             \hline
%         \end{tabular}
%     \end{minipage}%
%     \begin{minipage}{.5\linewidth}
%       \centering
%             \caption{AUC table.}\label{tab1}
%             \begin{tabular}{c|c|c|c}
            
%                  FC & Oper & AUC & No. param \\
%                 \hline
    
%                  - & Diff & 0.977 & 1.4M \\
%                  - & Concat & 0.520 & 1.4M \\
%                  128 & Diff & 0.978 & 4.5M \\
%                  128 & Concat & 0.594  & 4.5M \\
%                  256 & Diff & 0.981 & 8.7M \\
%                  256 & Concat & 0.949 & 8.7M \\
%                  512 & Diff & {\bfseries0.981} &  17.1M \\
%                  512 & Concat & 0.855 &  17.1M \\
%                  10284& Diff & 0.942 &  33.9M\\
%                  1024 & Concat & 0.968 &  33.9M\\
%             \hline
%             \end{tabular}
%     \end{minipage} 
% \end{table}


% and the challenge remains in the selection of an appropriate number of elements for the embedding. 
 works as initialization, defining the starting point for the optimization of the framework.

% The goal of this network is to extract a meaningful set of features that captures the overall appearance of the input structure.

% El encoder transforma la entrada en un vector de features 
Let $f_{\theta_{SE}}(\cdot)$ be an encoder function that extracts shape representation vectors from data examples $h_i^*=f_{\theta_{SE}}(x_i)$.
The encoder maps the data into a new space with meaningful information, where ideally, each value represents a shape characteristic. 

Let $g_{\theta_{SD}}(\cdot)$ be an encoder function that extracts shape representation vectors from data examples $h_i^*=f_{\theta_{SD}}(x_i)$.
The encoder maps the data into a new space with meaningful information, where ideally, each value represents a shape characteristic. 



% \begin{minipage}{\textwidth}
%     \begin{minipage}{.45\textwidth}
%         \centering
%         \resizebox{\textwidth}{!}{
%         \begin{tabular}{C{2cm}|c|C{1.5cm}|C{1.5cm}|C{1.5cm}||C{1.5cm}}
%             \hline
%             Backbone architecture & Siamese & Sagital flip & Merge operation & Num. params. & AUC (synthetic)  \\
%             \hline
%             LeNet & \xmark & \xmark & N/A & 5.4M & 0.62\\
%             LeNet & \cmark & \xmark & Diff. & 2.7M & 0.76 \\
%             LeNet & \cmark & \xmark & Concat. & 2.7M & 0.71 \\
%             LeNet & \cmark & \cmark & Diff. & 2.7M & {\bfseries0.99} \\
%             LeNet & \cmark & \cmark & Concat. & 2.7M & 0.73 \\
%             \hline
%             Deeper & \xmark & \xmark & N/A & 1.1M & 0.58 \\
%             Deeper & \cmark & \xmark & Diff. & 555K & 0.81 \\
%             Deeper & \cmark & \xmark & Concat. & 555K & 0.72 \\
%             Deeper & \cmark & \cmark & Diff. & 555K & 0.94 \\
%             Deeper & \cmark & \cmark & Concat. & 555K & 0.75 \\
%             \hline
%             \end{tabular}}
%     \end{minipage}%
% \hfill
% \begin{minipage}{.3\textwidth}
%     \centering
%     \includegraphics[width=1\textwidth]{miccaiAUC.pdf}
%     \label{fig:AUC}
% \end{minipage}
% \end{minipage}
@techreport{goubran2020hippocampal,
  title={Hippocampal segmentation for brains with extensive atrophy using three-dimensional convolutional neural networks},
  author={Goubran, Maged and Ntiri, Emmanuel Edward and Akhavein, Hassan and Holmes, Melissa and Nestor, Sean and Ramirez, Joel and Adamo, Sabrina and Ozzoude, Miracle and Scott, Christopher and Gao, Fuqiang and others},
  year={2020},
  institution={Wiley Online Library}
}





\author{Duilio~Deangeli\inst{1,2}%\orcidID{0000-1111-2222-3333} 
\and
Emmanuel~Iarussi\inst{2,3}
\and
Ignacio~Larrabide\inst{1,2}%\orcidID{1111-2222-3333-4444} 
\and
José~Ignacio~Orlando\inst{1,2}%\orcidID{0000--0001-9734-5571}
}
%
\authorrunning{D. Deangeli et al.}

\institute{Yatiris, PLADEMA, UNICEN, Tandil, Buenos Aires, Argentina \and
CONICET, Buenos Aires, Argentina \and
Universidad Torcuato Di Tella, CABA, Argentina}

% Furthermore, the volume was attached to the input image to debunk the hypothesis that the method only focuses on the volume.

% Hybrid models, which use a pretext task to generate features and a detection algorithm to classify normal from abnormal, showed good performance on synthetic data but were not as successful on real data tasks.
% \begin{table}[!htb]
%       \centering
%             \caption{AUC table for the different methods.}\label{AUC table}
% \resizebox{\textwidth}{!}{
%             \begin{tabular}{c|C{1.8cm}|C{1.5cm}|C{1.5cm}|C{1.5cm}|C{1.5cm}|C{1.5cm}}
%             \hline
%             \textbf{Method}  &  \textbf{Synthetic} & \textbf{MCI} & \textbf{AD (ADNI)} & \textbf{AD (OASIS)} & \textbf{HSL} & \textbf{HSR}\\
%             \hline
%             Absolute volume difference  & 0.72 & 0.56 & 0.55 & 0.62 & 0.95 & 0.94 \\
%             Normalized volumetric differences  & 0.75 & 0.58 & 0.62 & 0.64 & 0.95 & 0.94 \\
%             \hline
%             ShapeDNA + OC-SVM & 0.66 & 0.52 & 0.66 & 0.47 & 0.80 & 0.90 \\
%             ShapeDNA + HC shape features + OC-SVM & 0.93 & 0.59 & 0.67 & 0.65 & 0.92 & 0.98 \\
%             \hline
%             %LeNet-SiamAE + OC-SVM & 0.992 & 0.453 & 0.461 & & 0.658 & 0.666 \\
%             LeNet SiamAE + OC-SVM & {\bfseries0.99} & 0.43 & 0.46 & 0.45 & 0.78 & 0.74 \\
%             Deeper SiamAE + OC-SVM & 0.94 & 0.45 & 0.48 & 0.47 & 0.79 & 0.76 \\
%             \hline
%             \textbf{Deep NORHA (w/o CAE pretr.)} & 0.98 & {\bfseries0.98} & 0.99 & 0.87 & {\bfseries1} & {\bfseries1} \\
%             \textbf{Deep NORHA (with CAE pretr.)} & {\bfseries0.99} & {\bfseries0.98} & {\bfseries1} & \textbf{0.94} & {\bfseries1} & {\bfseries1} \\
%             \textbf{Deep NORHA + volume } & 0.80 & 0.62 & 0.72 & 0.62 & 0.99 & 0.98 \\
%             \hline
%             \end{tabular}}
% \end{table}

% \begin{table}[!htb]
%       \centering
%             \caption{AUC (95\% CI)  table for the different methods.}\label{AUC table}
% \resizebox{\textwidth}{!}{
%             \begin{tabular}{c|C{2.3cm}|C{2.3cm}|C{2.3cm}|C{2.3cm}|C{2.3cm}|C{2.3cm}}
%             \hline
%             \textbf{Method}  &  \textbf{Synthetic} & \textbf{MCI} & \textbf{AD (ADNI)} & \textbf{AD (OASIS)} & \textbf{HSL} & \textbf{HSR}\\
%             \hline
%             Absolute volume difference  & 0.72 (0.62-0.81) & 0.56 (0.46-0.66) & 0.55 (0.42-0.67) & 0.62 (0.51-0.74) & 0.95 (0.89-0.99) & 0.94 (0.82-1.00) \\
%             Normalized volumetric differences  & 0.82 (0.74-0.89) & 0.58 (0.48-0.68) & 0.62 (0.49-0.74) & 0.64 (0.53-0.74) & 0.95 (0.88-1.00) & 0.94 (0.83-1.00) \\
%             \hline
%             ShapeDNA + OC-SVM & 0.66 (0.56-0.74) & 0.52 (0.42-0.60) & 0.66 (0.55-0.76) & 0.47 (0.35-0.60) & 0.80 (0.69-0.90) & 0.90 (0.81-0.98) \\
%             ShapeDNA + HC shape features + OC-SVM & 0.93 (0.89-0.97) & 0.58 (0.49-0.66) & 0.67 (0.57-0.76) & 0.65 (0.53-0.77) & 0.92 (0.88-0.96) & 0.98 (0.95-1.00) \\
%             \hline
%             LeNet SiamAE + OC-SVM & 0.93 (0.88-0.97) & 0.48 (0.38-0.58) & 0.50 (0.37-0.61) & 0.46 (0.40-0.51) & 0.77 (0.67-0.86) & 0.69 (0.56-0.81)  \\
%             Deeper SiamAE + OC-SVM & 0.94 (0.90-0.98) & 0.45 (0.35-0.56) & 0.48 (0.35-0.59) & 0.47 (0.42-0.53) & 0.80 (0.69-0.88) & 0.76 (0.65-0.86) \\
%             \hline
%             \textbf{Deep NORHA (w/o CAE pretr.)} & 0.97 (0.95-0.99) & {\bfseries0.98} (0.95-1.00) & 0.99 (0.98-1.00) & 0.86 (0.82-0.91) & {\bfseries1.00} (1.00-1.00) & {\bfseries1.00} (1.00-1.00) \\
%             \textbf{Deep NORHA (with CAE pretr.)} & {\bfseries0.99} (0.99-1.00) & {\bfseries0.98} (0.95-1.00) & {\bfseries1.00} (0.99-1.00) & {\bfseries0.94} (0.91-0.97) & {\bfseries1.00} (1.00-1.00) & {\bfseries1.00} (1.00-1.00) \\
%             \textbf{Deep NORHA + volume } & 0.78 (0.70-0.87) & 0.62 (0.55-0.69) & 0.73 (0.64-0.80) & 0.62 (0.54-0.70) & 0.99 (0.97-1.00) & 0.98 {\scriptsize (0.96-1.00)} \\
%             \hline
%             \end{tabular}}
% \end{table}

% Además, se realizó un estudio de ablación para estudiar la influencia de ........ 
% To study the effect of depth in the model, we change the architecture of the encoder for a deeper one \cite{oktay2017anatomically}. 


%En este trabajo, proponemos un metodo novedoso para la caracterizacion automatica de asimetrias normales en estructuras homologas cerebrales basada en deteccion de anomalias y representation learning. El mismo se basa en una arquitectura siamesa formada por un encoder de forma que extrae caracteristicas relevantes que decriban la morfologia de las regiones izquierda y derecha de una determinada estructura cerebral. Las mismas se combinan mediante una APH, y ambos modulos son entrenados usando una estrategia combinada de self-supervised learning and Support Vector Data Description. El modelo solo se entrena usando normales, y dada un nuevo caso, permite obtener un indice de desviacion de asimetrias normales que es mas alto comforme mas se desvian de las capturadas en la poblacion sana de entrenamiento. Esto permite utilizarlo como una herramienta de diagnostico mas para la identificacion de condiciones neurodegenerativas. En pruebas realizadas para caraacterizar asimetrias normales entre hipocamos, el modelo propuesto demostro buenos resultados.







The parameters $\gamma$ and $\nu$ of the OC-SVM were adjusted using synthetic samples from $S_\text{all}$.

for asymmetry characterization and/or anomaly detection in the literature. 


In particular, we included: (i) the absolute and (ii) normalize volume difference used in \JIOc{XXX} to characterize hippocampal asymmetries; 


% Para comparar nuestro método se tomaron diversos baselines. (describir cada uno).
% -
% -
% -
% La configuración de cada uno. % Cada baseline, cómo se entrenó.
We select the following classification models for comparison:
\begin{enumerate}
    \item Absolute volume difference: This method uses the difference between volume directly as : \(vol^{diff} = \frac{vol^{left}-vol^{right}}{vol^{left}+vol^{right}}*100\), to classify normal of abnormal. A OC-SVM~\cite{scholkopf1999support} model was used as classifier and hyperparameters $\gamma$ and $\nu$ were adjusted using synthetic samples from $S_\text{all}$.
    \item Normalize volumetric difference: This method uses the same approach as above, but the data is normalize using mix-max strategy.
    \item Shape DNA + OC-SVM: Brainprint \cite{reuter2006laplace} is used with a OC-SVM to separate the normal and abnormal data points. Hyperparameters were adjusted by optimizing the F1-score for detecting pseudo anomalies artificially generated by manipulating the normal data on each of the validation folds as in \textcolor{red}{[cite]}. 
    \item NORHA: Same setting used in [paper NORHA].
    \item LeNet SiamAE + OC-SVM: LeNet architecture in the CAE for learning representations, and a OC-SVM as classifier to detect abnormal samples. Synthetic samples from $S_\text{all}$ were used to optimize the classifier parameters.
    \item Depper SiamAE + OC-SVM: This model was trained in the same way that LeNet above. However the CAE has the same setting as \cite{oktay2017anatomically}, which showed good results for 3D segmentation incorporating underlying anatomy knowledge.
    \item AD binary classification model: similar to ~\cite{li2021hippocampal} but using our architecture + a FC classification layer on top. It is trained with Cross Entropy objective function for Alzeimer's detection.
    \item Deep NORAH without CAE pretrained: The model is developed by the proposed method in this paper, where the encoder uses random initialization.
    \item Deep NORAH with CAE pretrained: In this case, the weights of trained CAE are used for the encoder initialization.
    %\item Deep NORAH + Volume: Same setting as mention above, but the volume is added in the input.
\end{enumerate}



%Distances of the NC subjects with respect to $\mathbf{c}$ are the lowest observed. 
%In the synthetic samples $S$, distances become larger as the deformation parameter $\sigma$ increases.  
%Cases with MCI are closer to the center than those with AD, which is consistent with medical observations.
%HSL and HSR cases, on the other hand, which are characterized by a significant atrophy on the left or right hippocampus, respectively, are the ones with the largest distances.
%-----
%As abnormal subjects deviate farther from the center than normal ones, we can study how the different diseases affect the general asymmetry. Figure~\ref{fig:boxplot} represents the distance of each test sample to the normal asymmetry center. In the validation set, it can be observed that the stronger the force, the farther the sample falls from the center. In the test set, the subjects with MCI are farther from the normal center but closer compared to the AD subjects. HSx, on the other hand, show a significantly greater distance from the normal center compared to all other test sets.

%Fig.~\ref{fig:boxplot_n_tsne} provides a $t$-SNE representation of the overall distribution of the embeddings. NC samples (green) are approximately together in the projection space, while MCI samples are close to NC from OASIS. AD cases are clustered together, with those from OASIS being closer to the ones from ADNI to the NC cases. Finally, HSL, HSR and synthetic cases altered with the largest $\sigma$ value are in the farthest regions with respect to the control ones. All these observations are consistent with what was previously seen in Fig.~\ref{fig:boxplot_n_tsne}.
%-----
%For further exploration of the results, a qualitative analysis was performed using the popular t-SNE technique. As shown in Figure~\ref{fig:TSNE}, well-clustered data was observed, providing useful insights into relationships between sets. It is noteworthy that the HSx sets were well separated from the rest of the sets. The NC groups of HEC and ADNI were also well isolated, while the NC OASIS was located at the bottom along with the MCI and AD samples.

